CosPGD: an efficient white-box adversarial attack for pixel-wise prediction tasks

While neural networks allow highly accurate predictions in many tasks, their lack of robustness towards even slight input perturbations often hampers their deployment. Adversarial attacks such as the seminal projected gradient descent (PGD) offer an effective means to evaluate a model's robustness and dedicated solutions have been proposed for attacks on semantic segmentation or optical flow estimation. While they attempt to increase the attack's efficiency, a further objective is to balance its effect, so that it acts on the entire image domain instead of isolated point-wise predictions. This often comes at the cost of optimization stability and thus efficiency. Here, we propose CosPGD, an attack that encourages more balanced errors over the entire image domain while increasing the attack's overall efficiency. To this end, CosPGD leverages a simple alignment score computed from any pixel-wise prediction and its target to scale the loss in a smooth and fully differentiable way. It leads to efficient evaluations of a model's robustness for semantic segmentation as well as regression models (such as optical flow, disparity estimation, or image restoration), and it allows it to outperform the previous SotA attack on semantic segmentation. We provide code for the CosPGD algorithm and example usage at https://github.com/shashankskagnihotri/cospgd.

==> figures/plots/deeplab_l2.tex <==
\begin{figure}[htb]
    \centering % <-- added
%\begin{subfigure}{0.49\textwidth}
%\caption{DeepLabV3 $l_2$-norm constrained}
\scriptsize DeepLabV3 $\ell_2$-norm constrained
  \includegraphics[width=\linewidth]{figures/plots/plot_deeplab_l2.pdf}
%  \label{plot:nontarget_l2:deeplab}
%\end{subfigure}
\caption{$\ell_2$-norm constrained CosPGD vs. PGD and SegPGD for semantic segmentation over PASCAL VOC2012 val set for DeepLabV3. See Appendix~\ref{subsec:exp_results:deeplabl2} for results for more $\alpha$ and $\epsilon$ values. \label{fig:nontarget_l2:deeplab}}%\vspace{-0.5em}
\vspace{1em}
\end{figure}

==> figures/plots/nontarget_l2.tex <==
\begin{figure}[htb]
    \centering % <-- added
\begin{subfigure}{0.49\textwidth}
\caption{DeepLabV3}
  \includegraphics[width=\linewidth]{figures/plots/deeplab_l2.pdf}
  
  \label{plot:nontarget_l2:deeplab}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.49\textwidth}
\caption{PSPNet}
  \includegraphics[width=\linewidth]{figures/plots/pspnet_l2.pdf}
  
  \label{plot:nontarget_l2:pspnet}
\end{subfigure}
\caption{Comparison of performance of CosPGD to PGD and SegPGD for semantic segmentation over PASCAL VOC2012 validation dataset as a $l_2$-norm constrained attack using DeepLabV3 in fig.\ref{plot:nontarget_l2:deeplab}  and PSPNet in fig.\ref{plot:nontarget_l2:pspnet}. We also report results as a table in the supplementary material. \label{fig:nontarget_l2}}
\end{figure}

==> tables/markdown.tex <==
\begin{tabular}{p{1.5cm}ccc|cc|cc|cc|cc|cc}
\toprule
 Network & Attack method & & & & & Attack iterations & & & & & & &\\
& & 3 & & 5 & & 10 & &  20 & &  40 & & 100 & \\
 &  & mIoU(\%) & mAcc(\%) &  mIoU(\%) & mAcc(\%) & mIoU(\%) & mAcc(\%) & mIoU(\%) & mAcc(\%) & mIoU(\%) & mAcc(\%)  & mIoU(\%) & mAcc(\%)\\
\midrule
UNet & SegPGD & 12.38 & 32.41 & 7.75 & 25.27 & 4.46 & 18.36  & 2.98  & 14.24 & 2.20 & 11.66 & 1.55 & 8.66 \\
  & CosPGD & 9.67  & 29.46 & 3.71 & 15.89  & 0.61 & 3.39 & 0.06 & 0.38 & 0.03 & 0.16 & 0.01 & 0.04 \\
\midrule
 PSPNet & PGD & 13.79 & 31.91 & 7.59 & 21.15 & 5.44 & 16.96 & 4.48 & 14.78  & 3.80  & 13.13 & 3.72 & 13.21  \\
  & SegPGD & 9.19 & 23.25 & 4.7 & 14.25 & 2.72 & 9.5 & 1.82 & 7.39  & 1.3  & 5.77 & 0.83 & 3.86  \\
 
  & CosPGD & 7.03  & 19.73 & 2.15 & 7.6 & 0.408 & 1.44 & 0.04 & 0.11 & 0.005 & 0.021 & 0.0002 & 0.0007 \\
  \midrule
DeepLabV3 & PGD & 10.69  & 28.76 & 8.0 & 25.29 & 7.02 & 24.05 & 6.84  & 23.87  & 6.79  &  23.81 & 7.01 & 24.13 \\
 
& SegPGD & 6.76  & 19.78 & 4.86 & 16.49 & 3.84 & 14.29 & 3.31  & 12.40  & 2.69  &  10.81 & 2.15 & 9.25 \\
 
  & CosPGD & 4.44  & 14.97 & 1.84 & 7.89 & 0.69 & 3.18 & 0.12 & 0.48 & 0.08 & 0.25 & 0.005 & 0.16 \\
\bottomrule

\end{tabular}

==> tables/pcfa_cospgd_l2.tex <==
%%%%%%%%%        NEW VALUES FOR ICLR   %%%%%%%%%%%%%%%%%%
\begin{table}[h]
\caption{Comparison of performance of CosPGD to PCFA as a targeted $l_2$-norm constrained attack for optical flow estimation over KITTI15 and Sintel validation datasets using different optical flow models over 3 random seeds. Average $epe$ values are compared, with respect to both, the \textbf{Target}  where a lower $epe$ indicates a better attack and \textbf{Initial flow prediction} (optical flow estimated by the model before any adversarial attack) where a higher $epe$ indicates a better attack. 
We compare over both targets used by \cite{pcfa}, i.e. zero vector ~$\overrightarrow{0}$ and Negative of the Initial Flow.
%CosPGD and PCFA performance is very comparable.
%This table will be included in Section~\ref{subsec:appendix:PCFA} upon acceptance.
}

\label{tbl:pcfa_cospgd}
\centering
%\small
\rotatebox{270}{
\scalebox{.33}{
\begin{tabular}{@{}p{1.5cm}cc|cc|cc|cc||cc|cc|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{4}{3cm}{\textbf{Model}} &  \multicolumn{8}{c}{\textbf{KITTI 2015}} &  \multicolumn{16}{c}{\textbf{MPI Sintel}} \\
 & & & & & & & & & \multicolumn{8}{c|}{\textbf{clean}}  & \multicolumn{8}{c}{\textbf{final}}\\

&  \multicolumn{4}{c}{Target $\overrightarrow{0}$} & \multicolumn{4}{c}{Negative Initial Flow} &  \multicolumn{4}{c}{Target $\overrightarrow{0}$} & \multicolumn{4}{c}{Negative Initial Flow} &  \multicolumn{4}{c}{Target $\overrightarrow{0}$} & \multicolumn{4}{c}{Negative Initial Flow} \\

 &  \multicolumn{2}{c}{wrt Target\textcolor{green}{$\downarrow$}} & \multicolumn{2}{c}{\textcolor{black}{wrt Initial\textcolor{green}{$\uparrow$}}} &  \multicolumn{2}{c}{wrt Target\textcolor{green}{$\downarrow$}} & \multicolumn{2}{c||}{wrt Initial\textcolor{green}{$\uparrow$}} &  \multicolumn{2}{c}{wrt Target\textcolor{green}{$\downarrow$}} & \multicolumn{2}{c}{\textcolor{black}{wrt Initial\textcolor{green}{$\uparrow$}}} &  \multicolumn{2}{c}{wrt Target\textcolor{green}{$\downarrow$}}  &  \multicolumn{2}{c|}{wrt Initial\textcolor{green}{$\uparrow$}} &  \multicolumn{2}{c}{wrt Target\textcolor{green}{$\downarrow$}} & \multicolumn{2}{c}{\textcolor{black}{wrt Initial\textcolor{green}{$\uparrow$}}} &  \multicolumn{2}{c}{wrt Target\textcolor{green}{$\downarrow$}}  &  \multicolumn{2}{c}{wrt Initial\textcolor{green}{$\uparrow$}} \\
 

& CosPGD & PCFA & CosPGD & PCFA & CosPGD & PCFA & CosPGD & PCFA &  CosPGD & PCFA & CosPGD & PCFA &  CosPGD & PCFA & CosPGD & PCFA & CosPGD & PCFA & CosPGD & PCFA& CosPGD & PCFA & CosPGD & PCFA \\
\midrule

GMA & 28.69 $\pm$ 0.12 &	28.67 $\pm$ 0.17&	3.89 $\pm$ 0.09&	3.89 $\pm$ 0.15 & 47.00 $\pm$ 0.40&	47.08 $\pm$ 0.69&	19.22 $\pm$ 0.53&	19.20 $\pm$ 0.57& 16.87 $\pm$ 0.14&	16.76 $\pm$ 0.11&	1.75 $\pm$ 0.15&	1.85 $\pm$ 0.10& 29.25 $\pm$ 0.38&	29.05 $\pm$ 0.38&	8.58 $\pm$ 0.34&	8.82 $\pm$ 0.37& 17.34 $\pm$ 0.07&	17.31 $\pm$ 0.11&	0.53 $\pm$ 0.07	0.54 $\pm$ 0.11&
32.11 $\pm$ 0.20&	32.04 $\pm$ 0.24&	4.57 $\pm$ 0.22&	4.64 $\pm$ 0.24\\

PWCNet & 19.13 $\pm$ 0.04	&18.96 $\pm$ 0.08	&3.25 $\pm$ 0.08&	3.47 $\pm$ 0.14 & 33.13 $\pm$ 0.25&	33.13 $\pm$ 0.26&	12.01 $\pm$ 0.20&	12.02 $\pm$ 0.22 & 12.20 $\pm$ 0.21 &	12.18 $\pm$ 0.07&	4.87 $\pm$ 0.17&	4.75 $\pm$ 0.12 & 20.57 $\pm$ 0.21&	20.43 $\pm$ 0.21&	13.20 $\pm$ 0.13&	13.21 $\pm$ 0.29 & 13.61 $\pm$ 0.10&	13.44 $\pm$ 0.14&	3.52 $\pm$ 0.13&	3.66 $\pm$ 0.12 & 23.00 $\pm$ 0.30&	23.01 $\pm$ 0.06&	10.84 $\pm$ 0.28&	10.75 $\pm$ 0.05 \\

RAFT & 29.09 $\pm$ 0.03&	29.17 $\pm$ 0.11&	3.75 $\pm$ 0.05&	3.63 $\pm$ 0.10 &  48.83 $\pm$ 0.35&	48.93 $\pm$ 0.29&	17.97 $\pm$ 0.29&	17.81 $\pm$ 0.27 & 16.42 $\pm$ 0.03&	16.46 $\pm$ 0.05&	1.69 $\pm$ 0.04&	1.65 $\pm$ 0.06 & 29.01 $\pm$ 0.11&	29.20 $\pm$ 0.01&	7.67 $\pm$ 0.11&	7.47 $\pm$ 0.05 & 17.38 $\pm$ 0.04&	17.36 $\pm$ 0.03&	0.55 $\pm$ 0.09&	0.50 $\pm$ 0.03 & 32.72 $\pm$ 0.22&	32.72 $\pm$ 0.14	& 3.71 $\pm$ 0.21&	3.75 $\pm$ 0.13 \\

SpyNet & 9.00 $\pm$ 0.01&	9.01 $\pm$ 0.03&	5.31 $\pm$ 0.01&	5.35 $\pm$ 0.06 & 12.10 $\pm$ 0.02&	12.08 $\pm$ 0.05&	16.47 $\pm$ 0.03&	16.44 $\pm$ 0.05 & 9.69 $\pm$ 0.01	&9.75 $\pm$ 0.07&	6.40 $\pm$ 0.05&	6.35 $\pm$ 0.00 & 13.08 $\pm$ 0.01&	13.17 $\pm$ 0.03&	18.75 $\pm$ 0.02&	18.76 $\pm$ 0.06 & 11.56 $\pm$ 0.01&	11.59 $\pm$ 0.03&	4.97 $\pm$ 0.01	& 4.97 $\pm$ 0.01 & 16.51 $\pm$ 0.01&	16.55 $\pm$ 0.06&	16.52 $\pm$ 0.01&	16.47 $\pm$ 0.05 \\
\bottomrule

\end{tabular}
}}
\end{table}
